Combining the Mersenne Twister and the Xorgens Designs

We combine the design of two \emph{random number generators}, \emph{Mersenne Twister} and \emph{Xorgens}, to obtain a new class of generators with heavy-weight characteristic polynomials (exceeded only by the {\sc well} generators) and high speed (comparable with the originals). Tables with parameter combinations are included for state sizes ranging from 521 to 44497 bits and each of the word lengths 32, 64, 128. These generators passed all tests of the \emph{TestU01}-package for each 32-bit integer part and each 64-bit derived real part of the output. We determine \emph{dimension gaps} for 32-bit words, neglecting the non-linear tempering, and compare with an alternative experimental linear tempering.

==> sc3 <==
%
% 
\section*{{Appendix: \sc mxg} C-code}
\label{S:C-code}
% 
\par
This section presents the core C-code of a generic 64-bit {\sc mxg}
which has been used for testing the speed of our generators
(we do not include a \texttt{main()}).
The definition of the lower and upper mask are derived from the column headed ``r''
in table \ref{S:MXGgenerators:T:designs64bit}.
For instance, \( M_{13} \) has \( r = 55 \).
The corresponding upper mask (UM) and lower mask (LM) are
\begin{verbatim}
#define UM 0xff80000000000000ULL // 9 bits at the left
#define LM 0x007fffffffffffffULL // 55 bits at the right
\end{verbatim}
Then add the definition of
\texttt{NN, MM, LA, RB, LC, RD} from the table.
The code for 128 bits requires a special header file (\texttt{emmintrin.h})
and some definitions of word operations: shift, xorshift, add.
Our code uses \texttt{inline} calls and
was compiled with~\texttt{gcc -03 -fno-strict-aliasing}~for a speedup.
N.B.: our {\sc xg} code used for speed measurement was derived from the present code
(not Brent's original code) to be comparable.
\bigskip
\begin{verbatim}
#define WLEN 64	// wordlength
#define WS 27	// shift combined with weyl generator
#define Weyl 0x61c8864680b583ebULL; // Weyl constant

static unsigned long long x[NN]; // state space
static int idx;		// state index
static unsigned long long w; // Weyl generator
static int hasWeyl = 1;	// Boolean

// include an explicit call of seed() in main()
void seed( unsigned long long s ) {
  unsigned long long v;
  int k;
  if ( !s ) s = 1ULL;
  for (k = WLEN; k > 0; k--) {
    s ^= s<<10; s ^= s>>15;
    s ^= s<<4;  s ^= s>>13;
  }
  for ( v = s, k = 0; k < NN; k++) {
    v ^= v<<10; v ^= v>>15;
    v ^= v<<4;  v ^= v>>13;
    x[k] = v + ( s += Weyl );
  }
  for (k = 4; k > 0; k--) nextstate(); // skip 4*NN calls
  idx = 0;
  w = s;
}	// seed, conforms with Brent's

inline void nextstate( ) {
  unsigned long long u, v;
  int i;
  for ( i = 0;  i < NN - MM; i++ ) {
    u = ( x[i] & UM ) | ( x[i+1] & LM );
    v = x[i+MM];
    u ^= u << LA;  u ^= u >> RB; // (I + LA)(I + RB)
    v ^= v << LC;  v ^= v >> RD; // (I + LC)(I + RD)
    x[i] = (v ^ u);
   }
  for ( ; i < NN - 1; i++ ) {
    u = ( x[i] & UM ) | ( x[i+1] & LM );
    v = x[i+MM-NN];
    u ^= u << LA;  u ^= u >> RB;
    v ^= v << LC;  v ^= v >> RD;
    x[i] = (v ^ u);
  }
  u = (x[NN-1] & UM) | (x[0] & LM);
  v = x[MM-1];
  u ^= u << LA;  u ^= u >> RB;
  v ^= v << LC;  v ^= v >> RD;
  x[NN-1] = (v ^ u);
}	// nextstate

// produce a 64-bit unsigned integer */
inline unsigned long long urand( ) {
  if ( ++idx >= NN) { nextstate(); idx = 0; }
  if ( hasWeyl ) {
    w += Weyl;
    return (x[idx] + (w ^ (w >> WS)));
  }
  return x[idx];
}	// urand

#define sr      11
// produce a real number in [0,1) based on 53 bits
inline double rrand( ) {
  double r;
  unsigned long long    u = 0ULL;
  static double scale = 1.0 / 9007199254740992.0;
  while ( !u ) u = urand( ) >> sr;
  r = (double) ( u - 1ULL );
  return scale * r;
}	// rrand
#undef sr
\end{verbatim}

